Re-Attention Transformer for Weakly Supervised Object Localization

Weakly supervised object localization is a challenging task which aims to localize objects with coarse annotations such as image categories. Existing deep network approaches are mainly based on class activation map, which focuses on highlighting discriminative local region while ignoring the full object. In addition, the emerging transformer-based techniques constantly put a lot of emphasis on the backdrop that impedes the ability to identify complete objects. To address these issues, we present a re-attention mechanism termed token refinement transformer (TRT) that captures the object-level semantics to guide the localization well. Specifically, TRT introduces a novel module named token priority scoring module (TPSM) to suppress the effects of background noise while focusing on the target object. Then, we incorporate the class activation map as the semantically aware input to restrain the attention map to the target object. Extensive experiments on two benchmarks showcase the superiority of our proposed method against existing methods with image category annotations. Source code is available in \url{https://github.com/su-hui-zz/ReAttentionTransformer}.

==> sections/sec-related.tex <==
\section{Related Work}
\subsection{CAM-based Attention Map Generation}
% A slew of approaches for weakly supervised object localization~\cite{zhang2021weakly} have been developed in the past decade. Among those approaches, a milestone work is 
The milestone work of the class activation map (CAM~\cite{zhou2016learning}) aims to localize the discriminative regions for a specific category. In this study, we grouped CAM techniques into two categories: activation-based approaches~\cite{zhou2016learning,wang2020score,wang2020ss,naidu2020cam,ramaswamy2020ablation} and gradient-based approaches~\cite{selvaraju2017grad,chattopadhay2018grad,omeiza2019smooth,fu2020axiom,jiang2021layercam}. Typical activation-based works dispose of the reliance on the gradient as they only require access to class activation map and the channel-wise confidence. 
%For example, Wang et al.~\cite{wang2020score} propose Score-CAM that computes the importance weights with the channel-wise increase of confidence performed on the activation map. Further, an extended version named SS-CAM~\cite{wang2020ss} provides better post-hoc explanations about the centralized target object in the image using smoothing to obtain a better understanding. In addition, other popular works, such as integrated score CAM (IS-CAM)~\cite{naidu2020cam}, attempt to alleviate the issue of saturation and false confidence and also achieve significant results. 
Apart from activation-based approaches, researchers often employ gradient information to enhance the salience of the image. Gradient-based methods highlight the important regions based on the back-propagated gradients of the specific class. 
%However, the naive Grad-CAM~\cite{selvaraju2017grad} often fails to localize objects in an image when multiple occurrences of the same category exist. Chattopadhyay et al. propose Grad-CAM++~\cite{chattopadhay2018grad} to overcome above issue by introducing pixel-wise weighting of the gradients of the output with respect to a particular region in the final feature map. Moreover, the work of smooth Grad-CAM++~\cite{omeiza2019smooth} combines both smoothing and Grad-CAM++~\cite{selvaraju2017grad} to enable either visualizing a layer, subset of feature maps, or subset of neurons within a feature map.
Many additional techniques, including XGrad-CAM~\cite{fu2020axiom}, LayerCAM~\cite{jiang2021layercam} and others, have also contributed to the field's progress and delivered favorable results.

\subsection{Transformer-based Attention Map Generation}
Vision transformer~\cite{dosovitskiy2020image} has attracted increasing attentions in recent studies, for example image classification~\cite{graham2021levit,liu2021swin,touvron2021training,wang2021pyramid,yuan2021tokens}, object detection~\cite{carion2020end,dai2021up,sun2021rethinking} and semantic segmentation~\cite{xie2021segformer}. However, vision transformers generate tokens by splitting an image into a series of ordered patches and computing global relations between tokens which inevitably introduces background noise. Existing works have made earlier attempts to explore the importance over tokens on fine-grained datasets~\cite{he2021transfg,wang2021feature} to alleviate the global issue. 
%He et al.~\cite{he2021transfg} propose a part selection module that integrate all attention weights of the transformer into an attention map for guiding the network to form discriminative tokens. Inspired by similar motivation that the classification token in the transformer layer pays more attention to the global information which yields poor explanations, Wang et al.~\cite{wang2021feature} propose a feature fusion transformer to aggregate the dominant tokens from each transformer layer to compensate for the local information. 
In addition, few studies have been proposed to facet the highlighting region~\cite{chen2022lctr,gao2021ts} based on both CAM and transformer. Despite the fact that solid numerical results have been achieved, the highlight regions still bring issues derived from both CAM and Transformer. 
\subsection{Weakly Supervised Object Localization}
Conventional works, such as \cite{li2016weakly,cinbis2016weakly} formulate the task of weakly supervised object localization (WSOL) as a multiple instance learning (MIL) problem. However the canonical approaches to the problem of MIL are typically initialization-sensitive which are prone to get stuck in local minimal with high generalization error. Thus many approaches~\cite{kumar2010self,deselaers2010localizing,cabral2014matrix, cinbis2016weakly,tang2017multiple, zhang2021weakly} attempt to obtain good initial values or to explore the refinement methods in post-processing. Recent there have been sufficient advancements in deep neural networks (DNNs) to cope with the challenging WSOL task, such as CAM-based~\cite{zhou2016learning,selvaraju2017grad} and transformer-based approaches~\cite{dosovitskiy2020image,graham2021levit,gao2021ts}. While in this work, we follow the trend to deal with the problems caused by global background noise and local discriminative regions with the proposed re-attention mechanism.

%\subsection{Vision Transformer}

==> tables/tab-sota-la.tex <==
\begin{minipage}{\textwidth}
\centering
\begin{minipage}[t]{0.48\textwidth}
%\subfigure[]
%{
\centering
    \fontsize{6.0}{8}\selectfont
        \begin{tabular}{c|c|c|c|c}
        \hline
        \multirow {2}{*}{Methods} & \multirow{2}{*}{Backbone} & \multicolumn{3}{c}{Loc.Acc} \\ 
        \cline{3-5}
        %\hline
        ~ & ~ & Top-1 & Top-5 & Gt-Known \\
        \hline
        CAM\cite{zhou2016learning} & VGG16 & 44.2 & 52.2 & 56.0 \\
        ADL\cite{choe2019attention} & VGG16 & 52.4 & - & 75.4 \\
        SPG\cite{zhang2018self} & VGG16 & 48.9 & 57.2 & 58.9 \\
        RCAM\cite{zhang2020rethinking}  & VGG16 & 59.0 & - & 76.3 \\
        SLT-Net\cite{guo2021strengthen} & VGG16 & 67.8 & - & 87.6 \\
        \hline
        CAM\cite{zhou2016learning} & GoogLeNet & 41.1 & 50.7 & 55.1 \\
        SPG\cite{zhang2018self} & GoogLeNet & 46.7 & 57.2 & - \\
        RCAM\cite{zhang2020rethinking}  & GoogLeNet & 53.0 & - & 70.0 \\
        ADL\cite{choe2019attention} & InceptionV3 & 53.0 & - & - \\
        I2C\cite{zhang2020inter} & InceptionV3 & 65.99 & 68.34 & 72.6 \\
        SLT-Net\cite{guo2021strengthen} & InceptionV3 & 66.1 & - & 86.5 \\
        \hline
        TS-CAM\cite{gao2021ts} & Deit-S & 71.3 & 83.8 & 87.7 \\
        TS-CAM\cite{gao2021ts} & Deit-B & 75.8 & 84.1 & 86.6 \\
        %\hline
        TRT(ours) & Deit-B & 75.8 & 87.5 & 90.4 \\
         \hline
        \end{tabular}
      
        %\vspace{2.5mm}
        %\caption{ Comparison of TRT with state-of-the-art methods on the CUB-200-2011\cite{wah2011caltech}(Localization Accuracy)}\label{tab:sota-cub-la}
        %\end{threeparttable}
%}
\end{minipage}
%\hspace{4mm}
\hfill
%\label{fig:lt}
\begin{minipage}[t]{0.48\textwidth}
%\subfigure[] 
%{
    \centering
    \fontsize{6.0}{8}\selectfont
        \begin{tabular}{c|c|c|c|c}
        \hline
        \multirow {2}{*}{Methods} & \multirow{2}{*}{Backbone} & \multicolumn{3}{c}{Loc.Acc} \\ 
        \cline{3-5}
        %\hline
        ~ & ~ & Top-1 & Top-5 & Gt-Known \\
        \hline
        CAM\cite{zhou2016learning} & VGG16 & 42.8 & 54.9 & 59.0 \\
        ADL\cite{choe2019attention} & VGG16 & 44.9 & - & - \\
        SPG\cite{zhang2018self} & InceptionV3 & 48.6 & 60.0 & 64.7 \\
        RCAM\cite{zhang2020rethinking}  & VGG16 & 44.6 & - & 60.7 \\
        SLT-Net\cite{guo2021strengthen} & VGG16 & 51.2 & 62.4 & 67.2 \\
        \hline
        CAM\cite{zhou2016learning} & InceptionV3 & 46.3 & 58.2 & 62.7 \\
        SPG\cite{zhang2018self} & InceptionV3 & 48.6 & 60.0 & 64.7 \\
        RCAM\cite{zhang2020rethinking}  & GoogLeNet & 50.6 & - & 64.4 \\
        ADL\cite{choe2019attention} & InceptionV3 & 48.7 & - & - \\
        I2C\cite{zhang2020inter} & InceptionV3 & 53.1 & 64.1 & 68.5 \\
        SLT-Net\cite{guo2021strengthen} & InceptionV3 & 55.7 & 65.4 & 67.6 \\
        \hline
        TS-CAM\cite{gao2021ts} & Deit-S & 53.4 & 64.3 & 67.6 \\
        %\hline
        TRT(ours)  & Deit-B & 56.0 & 65.6 & 68.2\\
        \hline
        \end{tabular}
        \vspace{2.5mm}
        %\caption{Comparison of TRT with state-of-the-art methods on the ILSVRC\cite{russakovsky2015imagenet}(Localization Accuracy)} \label{tab:sota-imagenet-la}
        %\end{threeparttable}
%}
\end{minipage}	
\end{minipage}

==> tables/tab-subtables.tex <==
\begin{table}[h]
\centering
\resizebox{0.9\linewidth}{!}{
\begin{minipage}[t]{\linewidth}
\subfigure[Table A]
{
% 	\begin{minipage}[t]{0.35\linewidth}
	\centering   
	 \begin{tabular}{c|c|c}
    \hline
    \multicolumn{3}{c}{CUB} \\
    \hline
    Methods & Backbone & MaxBoxAccV2 \\
    \hline
    CAM\cite{zhou2016learning} & VGG & 63.7 \\
    %SPG\cite{zhang2018self}  & VGG & 63.7 \\
    ADL\cite{choe2019attention} & VGG & 66.3\\
    \hline
    VITOL & Deit-B & 73.17 \\
    TS-CAM\cite{gao2021ts} & Deit-B & 76.74 \\
    \hline
    TRT(ours) & Deit-B & 81.59 \\
    \hline
    \end{tabular}
    
% 	\end{minipage}
	}
	%\hspace{4mm}
	\hfill
    %\label{fig:lt}
    \subfigure[Table B] 
{

% 	\begin{minipage}[t]{0.35\linewidth}
	%\centering     

	 \begin{tabular}{c|c|c}
    \hline
    \multicolumn{3}{c}{CUB} \\
    \hline
    Methods & Backbone & MaxBoxAccV2 \\
    \hline
    CAM\cite{zhou2016learning} & VGG & 63.7 \\
    %SPG\cite{zhang2018self}  & VGG & 63.7 \\
    ADL\cite{choe2019attention} & VGG & 66.3\\
    \hline
    VITOL & Deit-B & 73.17 \\
    TS-CAM\cite{gao2021ts} & Deit-B & 76.74 \\
    \hline
    TRT(ours) & Deit-B & 81.59 \\
    \hline
    \end{tabular}
    
% 	\end{minipage}
	}
	
    %\label{fig:lt}
    \caption{Two column}
    \end{minipage}
    }
\end{table}

==> tables/table-token-method.tex <==
%\renewcommand{\arraystretch}{1.5} % 控制行高
\begin{table}[tp]
    \centering
    %\fontsize{6.5}{8}\selectfont
        \begin{tabular}{c|c|c|c|c}
        \hline
        \multirow {2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{\emph{Loc.Acc}} \\ 
        \cline{3-4}
        %\hline
        ~ & ~ & Top-1 & Gt-Known \\
        \hline
        CUB-200-2011 & thresh(τ=0.65) & 58.2 & 75.4 \\
        CUB-200-2011 & topk(k=65) & 75.3 & - & 90.1 \\
        CUB-200-2011 & adaptive thresh(u=0.6) & 75.5 & 91.1 \\
        \hline
        ILSVRC & thresh(τ=0.05) & 54.2 & 66.9\\
        ILSVRC & topk(k=150) & 56 & 68.1 \\
        ILSVRC & adaptive thresh(u=0.95) & 58.8 & 70.7 \\
         \hline
        \end{tabular}
      
        \vspace{2.5mm}
        \caption{Experimental results of Token selection strategies for metrics of \emph{Loc.Acc}.}\label{tab:sota-cub-la}
        %\end{threeparttable}
\end{table}
